Affine Invariant Covariance Estimation for Heavy-Tailed Distributions

In this work we provide an estimator for the covariance matrix of a heavy-tailed multivariate distributionWe prove that the proposed estimator $\widehat{\mathbf{S}}$ admits an \textit{affine-invariant} bound of the form \[(1-\varepsilon) \mathbf{S} \preccurlyeq \widehat{\mathbf{S}} \preccurlyeq (1+\varepsilon) \mathbf{S}\]in high probability, where $\mathbf{S}$ is the unknown covariance matrix, and $\preccurlyeq$ is the positive semidefinite order on symmetric matrices. The result only requires the existence of fourth-order moments, and allows for $\varepsilon = O(\sqrt{\kappa^4 d\log(d/\delta)/n})$ where $\kappa^4$ is a measure of kurtosis of the distribution, $d$ is the dimensionality of the space, $n$ is the sample size, and $1-\delta$ is the desired confidence level. More generally, we can allow for regularization with level $\lambda$, then $d$ gets replaced with the degrees of freedom number. Denoting $\text{cond}(\mathbf{S})$ the condition number of $\mathbf{S}$, the computational cost of the novel estimator is $O(d^2 n + d^3\log(\text{cond}(\mathbf{S})))$, which is comparable to the cost of the sample covariance estimator in the statistically interesing regime $n \ge d$. We consider applications of our estimator to eigenvalue estimation with relative error, and to ridge regression with heavy-tailed random design.

==> M-bound.tex <==
\section{Proof of Eq.~\eqref{eq:M-bound}}
\label{sec:M-bound}
Given~$X \in \R^d$ satisfying~$\E[X] = 0$,~$\E[X \otimes X] = \S$, and the subgaussian moment growth condition
\begin{equation}
\label{ass:subgaussian-apx}
\E^{1/p} [|\lang X, u \rang|^{p}] \le  \bar\kappa \sqrt{p} \cdot \E^{1/2} [\lang X, u \rang^{2}], \quad \forall u \in \R^d, \;\; p \ge 2,
%\tag{SG}
\end{equation}
our goal is to prove the bound
\begin{equation}
\label{eq:M-bound-apx}
M_n := \E^{1/2} \left[\max_{1 \le i \le n} \|X_i \otimes X_i - \S\|^2\right] \le O(1)\bar \kappa^2 \tr(\S) \log(n+1),
\end{equation}
where~$X_1, ..., X_n$ are i.i.d.~copies of~$X$. 
We will use the following well-known result:
\begin{theorem}
\label{th:subg-quad}
Let $X \in \R^d$ be centered, satisfy~\eqref{ass:subgaussian-apx}, and let~$\E[X \otimes X] =\S$. Then with probability at least~$1-\delta$ it holds
\[
\|X\|^2 \le O(1) \bar\kappa^2 \left(\tr(\S) + \|\S\|_{\F} \sqrt{\log\left({1}/{\delta}\right)} + \|\S\| \log\left({1}/{\delta}\right)\right). 
% + \| \mu\|_\Ma^2 \left[ 1 + \frac{\|\Ma\|_\infty}{\|\Ma\|_2}\sqrt{\log(1/\delta)}\right],
\]
where~$\|\S\|_{\F}$ and~$\|\S\|$ are the Frobenius and spectral norms of~$\S$; note that both are upper-bounded by~$\tr(\S)$. 
\end{theorem}
This result is obtained from~\cite[Theorem~1]{hsu2012tail} by setting~$\mu = 0$ and using that the moment growth assumption~\eqref{ass:subgaussian-apx} is equivalent, when~$\E[X] = 0$, to the moment generating function assumption:
\[
\E\left[\exp\lang X,u \rang \right] \le \exp(\sigma \|u\|^2), \quad \forall u \in \R^d,
\]
in the sense that both hold simultaneously hold with~$\bar\kappa$ and~$\sigma$ related through a constant factor (see~\cite[Section~5.2.3]{vershynin2010introduction}).
Moreover, we note in passing that the result can be improved: the factor~$\bar \kappa \ge 1$ ahead of $\tr(\S)$ can be improved to~$1$ (note that~$\tr(\S) = \E[\|X\|^2]$); we do not give a proof of the improved result since Theorem~\ref{th:subg-quad} suffices for our purposes.

Returning to our task, note that we can bound~$\mu^2(X) := \|X \otimes X - \S\|^2$ by the triangle inequality:
\[
\mu^2(X) \le 2\|X \otimes X\|^2 + 2\|\S\|^2 \le 2\|X\|^4 + 2\|\S\|^2.
\]
Hence,~$M_n$ satisfies
\begin{equation}
\label{eq:M-decomposition}
M_n \le \E^{1/2} \left[\max_{1 \le i \le n} \mu^2(X_i)\right] \le \sqrt{2} \|\S\| + \sqrt{2}\E^{1/2} \left[\max_{1 \le i \le n} \|X_i\|^4 \right].
\end{equation}
Squaring the bound of Theorem~\ref{th:subg-quad}, and taking the union bound, we obtain that w.p.~$\ge 1-\delta$,
\[
\max_{1 \le i \le n} \|X_i\|^4 \le O(1) \bar \kappa^4 \tr(\S)^2 (1 + \sqrt{\log(n/\delta)})^4 \le O(1) \bar\kappa^4 \tr(\S)^2 \log^2((n+1)/\delta),
\]
where in the end we used that~$\log((n+1)/\delta) \ge O(1)$ for all~$\delta \in (0,1]$.
Applying the triangle inequality again, we arrive at 
\[
\max_{1 \le i \le n} \|X_i\|^4 \le O(1) \bar\kappa^4 \tr(\S)^2 \left[\log^2(n+1) + \log^2(1/\delta) \right],
\]
whence, noting that the left-hand side is a non-negative random variable,
\[
\E \left[\max_{1 \le i \le n} \|X_i\|^4\right] \le O(1)\bar\kappa^4 \tr(\S)^2 \left( \log^2(n+1) + \int_{0}^{+\infty} e^{-\sqrt{t}} \textup{d}t \right) \le O(1)\bar\kappa^4 \tr(\S)^2 \log^2(n+1).
\]
Plugging this into~\eqref{eq:M-decomposition}, and estimating~$\|\S\| \le \bar \kappa^2 \tr(\S)$ (recall that~$\bar\kappa \ge 1$), we arrive at~\eqref{eq:M-bound-apx}.
\hfill \qed

==> preamble-heavy-covariance.tex <==
\usepackage{fullpage}
\usepackage{amsmath,amsthm,amssymb,amsfonts}
\usepackage{dsfont}
\usepackage{mathrsfs}
%\usepackage{times}
% For citations
%\usepackage{natbib}
%\usepackage{fullpage}
%\usepackage{cmap}
\usepackage[dvipsnames]{xcolor}
\usepackage[colorlinks]{hyperref}
\hypersetup{
    linkcolor=red,
    citecolor=OliveGreen,
    filecolor=black,
    urlcolor=black,
}
% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
%\usepackage[draft]{graphicx}
\usepackage{graphicx}

\usepackage{algorithm,algorithmicx,caption,subcaption,graphicx,color}
\usepackage{algpseudocode}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% NEW MACROES BEFORE ALE'S SYNC %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{comment}
\renewcommand{\le}{\leqs}
\renewcommand{\ge}{\geqs}
\newcommand{\leqs}{\leqslant}
\newcommand{\geqs}{\geqslant}
\newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\la}{\lambda}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\newcommand{\To}{{\bfseries{to}\;}}
\newcommand{\Admissible}{\texttt{Admissible}}
\newcommand{\True}{\texttt{True}}
\newcommand{\False}{\texttt{False}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\Z}{\mathds{Z}}
\newcommand{\thetamin}{\theta_{\min}}
\newcommand{\thetamax}{\theta_{\max}}
\newcommand{\whj}{\wh \jmath}
\newcommand{\proofpoint}[1]{$\boldsymbol{{#1}^o}.$}
\newcommand{\F}{\textup{F}}
\newcommand{\Median}{\texttt{Median}}
%\newcommand{\kxi}{\kappa_{\textup{res}}}
\newcommand{\kresp}{\varkappa}
%\newcommand{\half}{\frac{1}{2}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% AND AFTER THE MERGE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\qed}{\qedsymbol}
\renewcommand{\le}{\leqs}
\renewcommand{\ge}{\geqs}
\renewcommand{\leq}{\leqs}
\renewcommand{\geq}{\geqs}
\renewcommand{\preceq}{\prccq}
\renewcommand{\succeq}{\succq}
\renewcommand{\epsilon}{\veps}
\newcommand{\cond}{\textrm{cond}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\q}{\mathtt{q}}


\usepackage{xfrac}
\usepackage{enumitem}
\def\Argmin{\mathop{\hbox{\rm Argmin}}}
\def\Argmax{\mathop{\hbox{\rm Argmax}}}
%\def\Var{{\boldsymbol \Psi}}
%\def\Varn{{{\boldsymbol \Psi}_n}}
\def\Var{{\He}}
\def\Varn{{\He}_n}
\def\k{\kappa}
\def\He{\mathbf{H}}
\def\Gr{\mathbf{G}}
\def\Ma{\mathbf{M}}
\def\Qu{\mathbf{Q}}
\def\Id{\mathbf{I}}
\def\csX{{\widetilde X}}
\def\cH{\mathcal{H}}
\def\s{\mathtt{s}}
\def\RE{\textup{RE}}
%\def\k{\varkappa}
\def\Rp{\R^{(+)}}
\def\vtheta{\vartheta}
\def\bPhi{\Phi_c}
\newcommand{\parl}{\mathbin{\!/\mkern-5mu/\!}}
\newcommand{\indic}{\mathds{1}}

% FB
\newcommand{\note}[1]{{\textbf{\color{red}#1}}}
\newcommand{\odima}[1]{{\textbf{\color{red}#1}}}

\newcommand{\Q}{\mathbf{Q}}
\newcommand{\A}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bPsi}{\boldsymbol{\Psi}}
\newcommand{\tO}{\wt{O}}
\newcommand{\WM}{\textup{WM}}
\newcommand{\lmin}{\lambda_{\min}}
\newcommand{\lmax}{\lambda_{\max}}
\renewcommand{\S}{{\mathbf S}}
\newcommand{\J}{{\mathbf J}}
\newcommand{\lam}{\lambda}

\newcommand{\B}{\mathfrak{B}}
\newcommand{\wt}{\widetilde}
\newcommand{\lsim}{\lesssim}
\newcommand{\gsim}{\gtrsim}
\newcommand{\lang}{\langle}
\newcommand{\rang}{\rangle}
\newcommand{\ud}{\textup{d}}
\newcommand{\R}{\mathds{R}}
\newcommand{\E}{\mathds{E}}
\newcommand{\T}{\top}
\newcommand{\half}{\tfrac{1}{2}}
\newcommand{\Pn}{\mathbf{P}}
\newcommand{\wh}{\widehat}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cSc}{{\mathcal{S}_c}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\bP}{\mathbf{P}}
%\newcommand{\Z}{\mathcal{Z}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\tr}{\textup{tr}}
\newcommand{\df}{\texttt{\textup{df}}}
\newcommand{\bb}{\texttt{\textup{b}}}
\newcommand{\Prob}{\mathds{P}}
\newcommand{\prccq}{\preccurlyeq}
\newcommand{\succq}{\succcurlyeq}
\newcommand{\GSC}{\textup{GSC}}
\newcommand{\En}{\E_{n}}
\newcommand{\dto}{\rightsquigarrow}
\newcommand{\deff}{d_{\text{eff}}}
\newcommand{\reff}{\mathtt{r}}
\newcommand{\eps}{\epsilon}
\newcommand{\veps}{\varepsilon}
\newcommand{\Exp}{\textup{Exp}}
\newcommand{\vphi}{\varphi}
\def\op{\textup{op}}
\def\nuc{\textup{nuc}}
\def\Extra{\texttt{Extra}}
\renewcommand\qedsymbol{$\blacksquare$}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cEc}{{{\mathcal{E}_0^c}}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\Distrib}{\mathscr{P}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\ind}{\mathds{1}}
\newcommand{\newtoread}[1]{{\color{blue}#1}}
\newcommand{\dimacorr}[2]{{\color{magenta}#2}}

\newtheorem{exercise}{Exercise}[section]
\newtheorem{example}{Example}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{fact}{Fact}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{problem}{Open Problem}[section]
%\newcommand{\thmlinebreak}{
%	\makeatletter
%	\leavevmode
%	\nobreaktrue
%	\makeatother}
\newtheorem{innercustomass}{Assumption}

\newenvironment{customass}[1]
{\renewcommand\theinnercustomass{#1}\innercustomass}
{\endinnercustomass}

%\newcommand{\assnumber}{} % initialize
%\newtheorem*{ass}{Assumption \assnumber}
%\newenvironment{customass}[1]
%  {\renewcommand{\assnumber}{#1}%
%   \begin{ass}}
%  {\end{ass}}

\newtheorem{definition}{Definition}[section]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% CLEVEREF STUFF %%%%%%%%%%%%%%%%%%%%
\usepackage{cleveref}
\crefname{assumption}{Assumption}{Assumptions}
\crefname{equation}{Eq.}{Eqs.}
\crefname{figure}{Fig.}{Figs.}
\crefname{table}{Table}{Tables}
\crefname{section}{Sec.}{Secs.}
\crefname{theorem}{Thm.}{Thms.}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{corollary}{Cor.}{Cors.}
\crefname{example}{Example}{Examples}
\crefname{appendix}{Appendix}{Appendixes}
\crefname{remark}{Remark}{Remark}
